Nurgle: Exacerbating Resource Consumption in Blockchain State Storage via MPT Manipulation

Blockchains, with intricate architectures, encompass various components, e.g., consensus network, smart contracts, decentralized applications, and auxiliary services. While offering numerous advantages, these components expose various attack surfaces, leading to severe threats to blockchains. In this study, we unveil a novel attack surface, i.e., the state storage, in blockchains. The state storage, based on the Merkle Patricia Trie, plays a crucial role in maintaining blockchain state. Besides, we design Nurgle, the first Denial-of-Service attack targeting the state storage. By proliferating intermediate nodes within the state storage, Nurgle forces blockchains to expend additional resources on state maintenance and verification, impairing their performance. We conduct a comprehensive and systematic evaluation of Nurgle, including the factors affecting it, its impact on blockchains, its financial cost, and practically demonstrating the resulting damage to blockchains. The implications of Nurgle extend beyond the performance degradation of blockchains, potentially reducing trust in them and the value of their cryptocurrencies. Additionally, we further discuss three feasible mitigations against Nurgle. At the time of writing, the vulnerability exploited by Nurgle has been confirmed by six mainstream blockchains, and we received thousands of USD bounty from them.

==> backup.tex <==
\begin{table*}[]
\centering
\caption{Practical and estimated time cost for $\dosattack{}$ to collide distinct lengths of desired prefix for an \dosformula{indexing}}
\label{tab_preiamges}
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{@{}l|l|l|c|c@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}Digits \\(nibbles)\end{tabular} & Crafted data (hex encoding) & $\dosformula{indexing}$ (hex encoding) & \begin{tabular}[c]{@{}l@{}}Practical\\ time cost\end{tabular} & \begin{tabular}[c]{@{}l@{}}Estimated\\ time cost\end{tabular} \\
\midrule
1 & 0x51b0e4b84afc9c7e935fd1c54409abda46ffff07 & 0x$\underline{1}$09999afd60b733da226a060260c2d9f165f0f33516c5a3230d2b9538ae197e7 & $\dosformula{<1s}$ & $\dosformula{<1s}$ \\
2 & 0x7c0caee5b72d0c71a090c6f02522e89acfffff07 & 0x$\underline{11}$fb9e6a64c5a7c23fb27d08e3d74ea1018fcb0c60d2010cca6c6654dd95e4b8 & $\dosformula{<1s}$ & $\dosformula{<1s}$ \\
3 & 0x8f5ea3c9db43de4143e5717f44dcb43e05d0fe07 & 0x$\underline{111}$0dc62b86ce4609e860381909da5480d46b2e90ea19c5afac287be805c234b & $\dosformula{<1s}$ & $\dosformula{<1s}$ \\
4 & 0xbd6f8cba28b4a0218d0aedbc820a27248ee4fe07 & 0x$\underline{1111}$65e10752633a1ab85c219c618d6c6e6259fdb7c8d2397df9cb72d16e4149 & $\dosformula{<1s}$ & $\dosformula{<1s}$ \\
5 & 0xfccedcfd14858e8b1baf9a497e99af468012b507 & 0x$\underline{11111}$0e0c5d11a713c428c42a03a5a7c55d66c0e61158ef13a63776b94d384d0 & $\dosformula{<1s}$ & $\dosformula{<1s}$ \\
6 & 0x58b91f9cb0ffacae5d95c9e80c373d264993cc06 & 0x$\underline{111111}$078c719cdc5abc2195b645a72ba7dd4d15b12ab9cce3361466c402df69 & $\dosformula{<1s}$ & $\dosformula{<1s}$ \\
7 & 0x89f25e63c12c48a95c22cd4b19585f337a805f06 & 0x$\underline{1111111}$06b6090ca5f7027a7539dc73173e26a35b28645b47d4878db6bbddd62 & $\dosformula{<1s}$ & $\dosformula{<1s}$ \\
8 & 0xa0f0722109f07edd76cc1d2b29cfbc0122ca2b06 & 0x$\underline{11111111}$ce35790ede4c97cc847e55c91c0b3063f5cb56ab6ab93ee76381fa6a & $\dosformula{<1s}$ & $\dosformula{2s}$ \\
9 & 0x97637e992f835689667a48a0731ce1ebb44dc006 & 0x$\underline{111111111}$0b3bf4ed6dc409fb20328970a0f23dac93761a4347fcd4c84dfe8cc & $\dosformula{43s}$ & $\dosformula{36s}$ \\
10 & 0x2f1033b78f8fb3c04259202793d2d89169326d02 & 0x$\underline{1111111111}$ce8bad4529bfef324c88454fe4e72c3cd3974c0249c9adc764802a & $\dosformula{7m}$ & $\dosformula{9.6m}$ \\
11 & 0x267a239f1986295e996358a79f57b473ae264d05 & 0x$\underline{11111111111}$00822f67e0319be36eb814ade0ca60c65c62b41641e889eb48ad8 & $\dosformula{2.6h}$ & $\dosformula{2.5h}$\\
12 & 0xd4dfd776a81fcdfa2d601f1efa31a2ad8c21fe06 & 0x$\underline{111111111111}$834eea3006374356f398b29f9b709272533e759348f0bb07aa11 & $\dosformula{1.5d}$ & $\dosformula{1.7d}$\\
13 & 0xdf04b72b67666a59ff30c06dd079f1850b36ba04 & 0x$\underline{1111111111111}$ca536d3de683a3ab986f631ee733132457eccc0d9a011aa9e55 & $\dosformula{23.5d}$ & $\dosformula{27.4d}$\\ \bottomrule
\end{tabular}
}
\end{table*}




We explore a novel attack surface in blockchain, i.e., the blockchain's state storage, which is commonly adopted by mainstream blockchain platforms. The state storage, based on Merkle Patricia Trie (MPT) structure, plays a crucial role in maintaining the state (e.g., the account balance) within the blockchain. 
Besides, we design \dosattack{}, a novel Denial-of-Service (DoS) attack towards the state storage, by exacerbating resource consumption to impair the blockchain's performance.
\dosattack{} is inspired by two observations while how blockchain modifies state in state storage, i.e., the flaw of the gas mechanism and the heavy burden of state maintenance,
Specifically, \dosattack{} manipulates the state storage by proliferating the intermediate nodes within the state storage of the MPT structure, forcing the blockchain to spend more resources on state maintenance and verification. 
We evaluate the impact of \dosattack{} by our formal models,
and demonstrate its 
damage
and consequences on 
mainstream
blockchain platforms. The implications of \dosattack{} extend beyond the performance degradation of blockchain, potentially leading to reduce trust in blockchain platforms 
and cryptocurrency value. 
We further discuss feasible mitigations against \dosattack{}.
At the time of writing, the vulnerability under \dosattack{} has been confirmed by several mainstream blockchains (e.g., Ethereum, Binance Smart Chain, Polygon, Optimism, Avalanche, and Ethereum Classic), and we received bug
bounty rewards from them.

